Towards Robust Numerical Question Answering: Diagnosing Numerical Capabilities of NLP Systems

Numerical Question Answering is the task of answering questions that require numerical capabilities. Previous works introduce general adversarial attacks to Numerical Question Answering, while not systematically exploring numerical capabilities specific to the topic. In this paper, we propose to conduct numerical capability diagnosis on a series of Numerical Question Answering systems and datasets. A series of numerical capabilities are highlighted, and corresponding dataset perturbations are designed. Empirical results indicate that existing systems are severely challenged by these perturbations. E.g., Graph2Tree experienced a 53.83% absolute accuracy drop against the ``Extra'' perturbation on ASDiv-a, and BART experienced 13.80% accuracy drop against the ``Language'' perturbation on the numerical subset of DROP. As a counteracting approach, we also investigate the effectiveness of applying perturbations as data augmentation to relieve systems' lack of robust numerical capabilities. With experiment analysis and empirical studies, it is demonstrated that Numerical Question Answering with robust numerical capabilities is still to a large extent an open question. We discuss future directions of Numerical Question Answering and summarize guidelines on future dataset collection and system design.

==> body/perturb_example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccl}
\hline
\textbf{Capability}                                                                         & \textbf{Perturbation} & \textbf{Example problem}                                                                                                                                                                                                                                                                                       \\ \hline
\multirow{5}{*}{\begin{tabular}{@{}c@{}}Number Value\\      Understanding\end{tabular}}  & Noise                 & \begin{tabular}[c]{@{}l@{}}\original{Original}: A room   is \original{12} feet long and \original{8} feet wide. \\      How much carpet does one need to cover the whole floor?\\      \perturbed{Perturbed}: A room is \perturbed{12.2} feet long and \perturbed{8.4} feet wide. \\      How much carpet does one need to cover the whole floor?\end{tabular}                      \\ \cline{2-3} 
                                                                                            & Distribution          & \begin{tabular}[c]{@{}l@{}}\original{Original}: A room is \original{12} feet long and \original{8} feet wide. \\      How much carpet does one need to cover the whole floor?\\      \perturbed{Perturbed}: A room is \perturbed{624} feet long and \perturbed{582} feet wide. \\      How much carpet does one need to cover the whole floor?\end{tabular}                        \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Surface-form\\      Recognizing\end{tabular}}    & Language              & \begin{tabular}[c]{@{}l@{}}\original{Original}: A room   is \original{12} feet long and \original{8} feet wide. \\      How much carpet does one need to cover the whole floor?\\      \perturbed{Perturbed}: A room is \perturbed{twelve} feet long and \perturbed{eight} feet wide. \\      How much carpet does one need to cover the whole floor?\end{tabular}                  \\ \cline{2-3} 
                                                                                            & Type                  & \begin{tabular}[c]{@{}l@{}}\original{Original}: A room is \original{12} feet long and \original{8} feet wide. \\      How much carpet does one need to cover the whole floor?\\      \perturbed{Perturbed}: A room is \perturbed{12.0} feet long and \perturbed{8.0} feet wide. \\      How much carpet does one need to cover the whole floor?\end{tabular}                      \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Related Value\\      Selection\end{tabular}} & Verbosity             & \begin{tabular}[c]{@{}l@{}}\original{Original}: A room is \original{12} feet long and \original{8} feet wide. \\      How much carpet does one need to cover the whole floor?\\      \perturbed{Perturbed}: A room is \perturbed{12 (instead of 3)} feet long and \perturbed{8 (not 5)} feet wide.   \\      How much carpet does one need to cover the whole floor?\end{tabular}                                    \\ \cline{2-3} 
                                                                                            & Extra             & \begin{tabular}[c]{@{}l@{}}\original{Original}: \original{A room   is 12 feet long and 8 feet wide.} \\      How much carpet does one need to cover the whole floor?\\      \perturbed{Perturbed}: \perturbed{A room is 12 feet long and 8 feet wide. Jennie has 5 pens.} \\      How much carpet does one need to cover the whole floor?\end{tabular} 
                                                                                \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Logic Pattern \\ Recognizing\end{tabular}} & Operation             & \begin{tabular}[c]{@{}l@{}}\original{Original}: A room   is 12 feet long and 8 feet wide. \\      \original{How much carpet does one need to cover the whole floor?}\\     \perturbed{Perturbed}: A room is 12 feet long and 8 feet wide.   \\\perturbed{How much longer is the length than the width?}\end{tabular}                                    \\ \cline{2-3} 
                                                                                            & Order             & \begin{tabular}[c]{@{}l@{}}\original{Original}: A room   is \original{12 feet long} and \original{8 feet wide}. \\      How much carpet does one need to cover the whole floor?\\      \perturbed{Perturbed}: A room is \perturbed{8 feet wide} and \perturbed{12 feet long}. \\      How much longer is the length than the width?\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Examples of perturbed problems}
\label{tab:perturbed_examples}
\end{table*}

==> body/table_atk_asdiv-a.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{model} & \textbf{perturbation} & \textbf{eq\_acc} & \textbf{ans\_acc} & \textbf{$\Delta$ eq\_acc} & \textbf{$\Delta$ ans\_acc} \\ \midrule
BART & lang & 43.44\% & 45.90\% & \cellcolor[HTML]{C4DDB3}-20.49\% & \cellcolor[HTML]{BFDAAD}-22.13\% \\
BART & verbosity & 41.80\% & 43.44\% & \cellcolor[HTML]{BFDAAD}-22.13\% & \cellcolor[HTML]{B8D6A4}-24.59\% \\
BART & distri & 37.70\% & 54.92\% & \cellcolor[HTML]{B3D39E}-26.23\% & \cellcolor[HTML]{D9E9CE}-13.11\% \\
BART & noise & 48.36\% & 51.64\% & \cellcolor[HTML]{D2E5C5}-15.57\% & \cellcolor[HTML]{D0E4C2}-16.39\% \\
BART & type & 34.43\% & 57.38\% & \cellcolor[HTML]{AACE92}-29.51\% & \cellcolor[HTML]{E0EDD7}-10.66\% \\
BART & extra & 25.41\% & 27.05\% & \cellcolor[HTML]{90BF71}-38.52\% & \cellcolor[HTML]{89BB68}-40.98\% \\
BART & order & 33.61\% & 68.85\% & \cellcolor[HTML]{A8CD8F}-30.33\% & \cellcolor[HTML]{FFFFFF}0.82\% \\
BART & op & 30.33\% & 37.70\% & \cellcolor[HTML]{9EC783}-33.61\% & \cellcolor[HTML]{A8CD8F}-30.33\% \\
BART & original & 63.93\% & 68.03\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \midrule
T5 & lang & 49.18\% & 54.10\% & \cellcolor[HTML]{C9E0B9}-18.85\% & \cellcolor[HTML]{C9E0B9}-18.85\% \\
T5 & verbosity & 26.23\% & 28.69\% & \cellcolor[HTML]{87BA65}-41.80\% & \cellcolor[HTML]{80B65C}-44.26\% \\
T5 & distri & 51.64\% & 58.20\% & \cellcolor[HTML]{D0E4C2}-16.39\% & \cellcolor[HTML]{D4E6C8}-14.75\% \\
T5 & noise & 31.15\% & 36.07\% & \cellcolor[HTML]{95C277}-36.89\% & \cellcolor[HTML]{95C277}-36.89\% \\
T5 & type & 30.33\% & 61.48\% & \cellcolor[HTML]{93C174}-37.70\% & \cellcolor[HTML]{DEECD4}-11.48\% \\
T5 & extra & 42.62\% & 45.08\% & \cellcolor[HTML]{B6D5A1}-25.41\% & \cellcolor[HTML]{AFD198}-27.87\% \\
T5 & order & 33.61\% & 67.21\% & \cellcolor[HTML]{9CC680}-34.43\% & \cellcolor[HTML]{EEF5E9}-5.74\% \\
T5 & op & 38.52\% & 45.08\% & \cellcolor[HTML]{AACE92}-29.51\% & \cellcolor[HTML]{AFD198}-27.87\% \\
T5 & original & 68.03\% & 72.95\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \midrule
GPT2 & lang & 31.97\% & 32.79\% & \cellcolor[HTML]{DBEAD1}-12.30\% & \cellcolor[HTML]{DBEAD1}-12.30\% \\
GPT2 & verbosity & 33.61\% & 33.61\% & \cellcolor[HTML]{E0EDD7}-10.66\% & \cellcolor[HTML]{DEECD4}-11.48\% \\
GPT2 & distri & 31.15\% & 31.97\% & \cellcolor[HTML]{D9E9CE}-13.11\% & \cellcolor[HTML]{D9E9CE}-13.11\% \\
GPT2 & noise & 34.43\% & 36.07\% & \cellcolor[HTML]{E2EEDA}-9.84\% & \cellcolor[HTML]{E5F0DD}-9.02\% \\
GPT2 & type & 27.05\% & 34.43\% & \cellcolor[HTML]{CDE2BF}-17.21\% & \cellcolor[HTML]{E0EDD7}-10.66\% \\
GPT2 & extra & 15.57\% & \cellcolor[HTML]{FFFFFF}16.39\% & \cellcolor[HTML]{ACCF95}-28.69\% & \cellcolor[HTML]{ACCF95}-28.69\% \\
GPT2 & order & 16.39\% & 37.70\% & \cellcolor[HTML]{AFD198}-27.87\% & \cellcolor[HTML]{E9F2E3}-7.38\% \\
GPT2 & op & 18.85\% & 21.31\% & \cellcolor[HTML]{B6D5A1}-25.41\% & \cellcolor[HTML]{BBD8A7}-23.77\% \\
GPT2 & original & 44.26\% & 45.08\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \midrule
Graph2Tree & lang & 59.29\% & 61.20\% & \cellcolor[HTML]{E9F2E2}-7.65\% & \cellcolor[HTML]{E9F2E3}-7.38\% \\
Graph2Tree & verbosity & 33.61\% & 34.70\% & \cellcolor[HTML]{9FC884}-33.33\% & \cellcolor[HTML]{9EC782}-33.88\% \\
Graph2Tree & distri & 60.38\% & 62.02\% & \cellcolor[HTML]{ECF4E6}-6.56\% & \cellcolor[HTML]{ECF4E6}-6.56\% \\
Graph2Tree & noise & 67.21\% & 69.13\% & \cellcolor[HTML]{FFFFFF}0.27\% & \cellcolor[HTML]{FFFFFF}0.55\% \\
Graph2Tree & type & 67.21\% & 69.67\% & \cellcolor[HTML]{FFFFFF}0.27\% & \cellcolor[HTML]{FFFFFF}1.09\% \\
Graph2Tree & extra & 13.11\% & 13.93\% & \cellcolor[HTML]{70AD47}-53.83\% & \cellcolor[HTML]{70AD47}-54.64\% \\
Graph2Tree & order & 33.61\% & 61.48\% & \cellcolor[HTML]{9FC884}-33.33\% & \cellcolor[HTML]{EAF3E4}-7.10\% \\
Graph2Tree & op & 38.52\% & 46.72\% & \cellcolor[HTML]{ADD096}-28.42\% & \cellcolor[HTML]{C0DBAE}-21.86\% \\
Graph2Tree & original & 66.94\% & 68.58\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \bottomrule
\end{tabular}%
}
\caption{Attack Results on ASDiv-a}
\label{tab:atk_asdiv-a}
\end{table}

==> body/table_atk_drop-n.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{model} & \textbf{perturbation} & \textbf{ans\_acc} & \textbf{$\Delta$ ans\_acc} \\ \midrule
BART & lang & 35.62\% & \cellcolor[HTML]{D7E8CC}-13.80\% \\
BART & verbosity & 37.04\% & \cellcolor[HTML]{DBEAD1}-12.38\% \\
BART & type & 39.30\% & \cellcolor[HTML]{E2EED9}-10.13\% \\
BART & original & 49.42\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \midrule
T5 & lang & 38.80\% & \cellcolor[HTML]{E2EEDA}-9.88\% \\
T5 & verbosity & 39.84\% & \cellcolor[HTML]{E5F0DE}-8.84\% \\
T5 & type & 41.72\% & \cellcolor[HTML]{EBF3E5}-6.97\% \\
T5 & original & 48.68\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \bottomrule
\end{tabular}%
}
\caption{Attack results on DROP-n}
\label{tab:atk_drop-n}
\end{table}

==> body/table_atk_tatqa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{model} & \textbf{perturbation} & \textbf{EM} & \textbf{F1} & \textbf{$\Delta$ EM} & \textbf{$\Delta$ F1} \\ \midrule
TagOps & lang & 23.79\% & 23.79\% & \cellcolor[HTML]{A6CC8C}-18.62\% & \cellcolor[HTML]{A6CC8C}-18.62\% \\
TagOps & op & 28.12\% & 28.12\% & \cellcolor[HTML]{BAD7A7}-14.29\% & \cellcolor[HTML]{BAD7A7}-14.29\% \\
TagOps & type & 37.07\% & 37.07\% & \cellcolor[HTML]{E5F0DE}-5.34\% & \cellcolor[HTML]{E5F0DE}-5.34\% \\
TagOps & verbosity & 40.52\% & 40.52\% & \cellcolor[HTML]{F5F9F3}-1.90\% & \cellcolor[HTML]{F5F9F3}-1.90\% \\
TagOps & original & 42.41\% & 42.41\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \bottomrule
\end{tabular}%
}
\caption{Attack Results on TATQA}
\label{tab:atk_tat}
\end{table}

==> body/table_def_asdiv-a.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{model} & \textbf{perturbation} & \textbf{eq\_acc} & \textbf{val\_acc} & \textbf{$\Delta$ eq\_acc} & \textbf{$\Delta$ val\_acc} \\ \midrule
Graph2Tree & lang & 59.29\% & 61.20\% & \cellcolor[HTML]{C8DFB8}-7.65\% & \cellcolor[HTML]{CAE0BB}-7.38\% \\
Graph2Tree & verbosity & 66.67\% & 69.67\% & \cellcolor[HTML]{FDFDFC}-0.27\% & \cellcolor[HTML]{FFFFFF}1.09\% \\
Graph2Tree & distri & 60.11\% & 62.57\% & \cellcolor[HTML]{CEE2C0}-6.83\% & \cellcolor[HTML]{D4E6C7}-6.01\% \\
Graph2Tree & noise & 67.49\% & 68.85\% & \cellcolor[HTML]{FFFFFF}0.55\% & \cellcolor[HTML]{FFFFFF}0.27\% \\
Graph2Tree & type & 68.58\% & 70.49\% & \cellcolor[HTML]{FFFFFF}1.64\% & \cellcolor[HTML]{FFFFFF}1.91\% \\
Graph2Tree & original & 66.94\% & 68.58\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \midrule
T5 & verbosity & 52.46\% & 56.56\% & \cellcolor[HTML]{8FBF6F}-15.57\% & \cellcolor[HTML]{89BB68}-16.39\% \\
T5 & distri & 47.54\% & 52.46\% & \cellcolor[HTML]{70AD47}-20.49\% & \cellcolor[HTML]{70AD47}-20.49\% \\
T5 & type & 56.56\% & 60.66\% & \cellcolor[HTML]{ACCF95}-11.48\% & \cellcolor[HTML]{A7CC8D}-12.30\% \\
T5 & noise & 53.28\% & 58.20\% & \cellcolor[HTML]{95C277}-14.75\% & \cellcolor[HTML]{95C277}-14.75\% \\
T5 & lang & 55.74\% & 59.02\% & \cellcolor[HTML]{A7CC8D}-12.30\% & \cellcolor[HTML]{9BC57E}-13.93\% \\
T5 & original & \multicolumn{1}{l}{68.03\%} & \multicolumn{1}{l}{72.95\%} & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \midrule
BART & verbosity & 61.48\% & 65.57\% & \cellcolor[HTML]{D5E7CA}-5.74\% & \cellcolor[HTML]{CAE0BB}-7.38\% \\
BART & lang & 47.54\% & 48.36\% & \cellcolor[HTML]{72AE4A}-19.67\% & \cellcolor[HTML]{70AD47}-24.59\% \\
BART & type & 62.30\% & 66.39\% & \cellcolor[HTML]{DBEAD1}-4.92\% & \cellcolor[HTML]{D0E4C2}-6.56\% \\
BART & noise & 63.93\% & 68.03\% & \cellcolor[HTML]{E7F1E0}-3.28\% & \cellcolor[HTML]{DBEAD1}-4.92\% \\
BART & distri & 59.02\% & 63.11\% & \cellcolor[HTML]{C4DDB3}-8.20\% & \cellcolor[HTML]{B8D6A4}-9.84\% \\
BART & original & \multicolumn{1}{l}{67.21\%} & \multicolumn{1}{l}{72.95\%} & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \bottomrule
\end{tabular}%
}
\caption{Defense results on ASDiv-a}
\label{tab:def_asdiv-a}
\end{table}

==> body/table_def_drop-num.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{model} & \textbf{perturbation} & \textbf{ans\_acc} & \textbf{$\Delta$ ans\_acc} \\ \midrule
BART & original & 50.36\% & \cellcolor[HTML]{FFFFFF}0.00\% \\
BART & lang & 49.49\% & \cellcolor[HTML]{F8FBF7}-0.86\% \\
BART & type & 49.88\% & \cellcolor[HTML]{FBFDFA}-0.47\% \\
BART & verbosity & 44.29\% & \cellcolor[HTML]{D3E6C7}-6.06\% \\ \midrule
T5 & original & 49.52\% & \cellcolor[HTML]{F9FBF7}-0.83\% \\
T5 & lang & 48.52\% & \cellcolor[HTML]{F1F7EE}-1.84\% \\
T5 & type & 49.41\% & \cellcolor[HTML]{F8FBF6}-0.95\% \\
T5 & verbosity & 48.52\% & \cellcolor[HTML]{F1F7EE}-1.84\% \\ \bottomrule
\end{tabular}%
}
\caption{Defense results on DROP-num}
\label{tab:def_drop-num}
\end{table}

==> body/table_def_tatqa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{model} & \textbf{perturbation} & \textbf{EM} & \textbf{F1} & \textbf{$\Delta$ EM} & \textbf{$\Delta$ F1} \\ \midrule
TagOps & verbosity & 44.67\% & 52.89\% & \cellcolor[HTML]{E3EFDC}-5.68\% & \cellcolor[HTML]{E3EFDB}-5.77\% \\
TagOps & type & 39.27\% & 48.51\% & \cellcolor[HTML]{CAE0BB}-11.08\% & \cellcolor[HTML]{CEE3C0}-10.16\% \\
TagOps & lang & 42.24\% & 50.46\% & \cellcolor[HTML]{D8E8CD}-8.10\% & \cellcolor[HTML]{D7E8CC}-8.21\% \\
TagOps & original & 50.35\% & 58.67\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% \\ \bottomrule
\end{tabular}%
}
\caption{Defense results on TATQA}
\label{tab:def_tatqa}
\end{table}

==> body/table_drop.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{@{}cc|cc@{}}
\toprule
\multicolumn{2}{c|}{} &  &  \\
\multicolumn{2}{c|}{\multirow{-2}{*}{Configuration}} & \multirow{-2}{*}{T5} & \multirow{-2}{*}{BART} \\ \midrule
Setting & Perturbation & Acc\_ans & Acc\_ans \\ \midrule
 & Language & \cellcolor[HTML]{CFE0F3}35.62\% & \cellcolor[HTML]{CCDFF2}35.62\% \\
 & Type & \cellcolor[HTML]{DBE8F6}39.30\% & \cellcolor[HTML]{D8E6F5}39.30\% \\
\multirow{-3}{*}{Attack} & Verbosity & \cellcolor[HTML]{D3E3F4}37.04\% & \cellcolor[HTML]{D1E2F3}37.04\% \\ \midrule
 & Language & \cellcolor[HTML]{FCFCFF}49.49\% & \cellcolor[HTML]{F6F8FD}48.52\% \\
 & Type & \cellcolor[HTML]{FCFCFF}49.88\% & \cellcolor[HTML]{F8FAFE}49.41\% \\
\multirow{-3}{*}{Defense} & Verbosity & \cellcolor[HTML]{EBF1FA}44.29\% & \cellcolor[HTML]{F6F8FD}48.52\% \\ \midrule
Original & None & \cellcolor[HTML]{FCFCFF}49.42\% & \cellcolor[HTML]{FCFCFF}50.36\% \\ \bottomrule
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}
